Cooperative Deep $Q$-learning Framework for Environments Providing Image Feedback

In this paper, we address two key challenges in deep reinforcement learning setting, sample inefficiency and slow learning, with a dual NN-driven learning approach. In the proposed approach, we use two deep NNs with independent initialization to robustly approximate the action-value function in the presence of image inputs. In particular, we develop a temporal difference (TD) error-driven learning approach, where we introduce a set of linear transformations of the TD error to directly update the parameters of each layer in the deep NN. We demonstrate theoretically that the cost minimized by the error-driven learning (EDL) regime is an approximation of the empirical cost and the approximation error reduces as learning progresses, irrespective of the size of the network. Using simulation analysis, we show that the proposed methods enables faster learning and convergence and requires reduced buffer size (thereby increasing the sample efficiency).

==> references.tex <==
%%%%%%%%%%%%%%%%%%%%%%%% referenc.tex %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% sample references
% %
% Use this file as a template for your own input.
%
%%%%%%%%%%%%%%%%%%%%%%%% Springer-Verlag %%%%%%%%%%%%%%%%%%%%%%%%%%
%
% BibTeX users please use
%\bibliographystyle{unsrt}
%\bibliography{Refer.bib}

%\bibliographystyle{}
%\bibliography{}
%
\begin{thebibliography}{10}

\bibitem{Hespanha_NCS}
J.~P. {Hespanha}, P.~{Naghshtabrizi}, and Y.~{Xu}, ``A survey of recent results
  in networked control systems,'' {\em Proceedings of the IEEE}, 95:138--162, Jan 2007.

\bibitem{antsaklis2007special}
P.~Antsaklis and J.~Baillieul, ``Special issue on technology of networked
  control systems,'' {\em Proceedings of the IEEE}, 95(1): 5--8,2007.

\bibitem{Antsaklis2004TAC}
L.~A. {Montestruque} and P.~{Antsaklis}, ``Stability of model-based networked
  control systems with time-varying transmission times,'' 
  {\em IEEE Transactions on Automatic Control}, 49(9):1562--1572, 2004.

\bibitem{Sahoo2017}
A.~{Sahoo} and S.~{Jagannathan}, ``Stochastic optimal regulation of nonlinear
  networked control systems by using event-driven adaptive dynamic
  programming,'' {\em IEEE Transactions on Cybernetics}, 47(2):425--438, 2017.

\bibitem{wu2007design}
J.~Wu and T.~Chen, ``Design of networked control systems with packet
  dropouts,'' {\em IEEE Transactions on Automatic control}, 52(7):1314--1319, 2007.

\bibitem{HaoAutomatica}
H.~Xu, S.~Jagannathan, and F.~Lewis, ``Stochastic optimal control of unknown
  linear networked control system in the presence of random delays and packet
  losses,'' {\em Automatica}, 48(6):1017 -- 1030, 2012.

%\bibitem{Moghadam2019CYBER}
%R. Moghadam and H. Modares
%\newblock Resilient Autonomous Control of Distributed Multi-agent Systems in Contested Environments.
%\newblock {\em IEEE Transactions on Cybernetics}, 49(11):3957--3967, 2019. and attacks \cite{Moghadam2019CYBER} 
%%%%%%%%%%%%%%%%%% Time delay papers%%%%%%%%%%%%%%%%%
\bibitem{gu2003stability}
Keqin Gu, Jie Chen, and Vladimir~L Kharitonov.
\newblock {\em Stability of time-delay systems}.
\newblock Springer Science \& Business Media, 2003.

\bibitem{fridman2014Book}
Emilia Fridman.
\newblock {\em Introduction to Time-delay Systems: Analysis and C ontrol}.
\newblock Springer, 2014.

\bibitem{RICHARD20031667}
Jean-Pierre Richard.
\newblock Time-delay systems: an overview of some recent advances and open
  problems.
\newblock {\em Automatica}, 39(10):1667 -- 1694, 2003.

\bibitem{karafyllis2016recent}
Iasson Karafyllis, Michael Malisoff, Frederic Mazenc, and Pierdomenico Pepe.
\newblock Recent results on nonlinear delay control systems.
\newblock {\em Springer International Publishing Switzerland}, 2016.

\bibitem{ZhuKrstic2017TAC}
Y. Zhu and M. Krstic and H. Su
\newblock Adaptive Output Feedback Control for Uncertain Linear Time-Delay Systems.
\newblock {\em IEEE Transactions on Automatic Control}, 62(2):545--560, 2017.

\bibitem{Ponomarev2016TAC}
A. Ponomarev
\newblock Reduction-Based Robustness Analysis of Linear Predictor Feedback for Distributed Input Delays.
\newblock {\em IEEE Transactions on Automatic Control}, 61(2):468--472, 2016.

\bibitem{Artstein1982TAC}
Z. Artstein
\newblock Linear systems with delayed controls: A reduction.
\newblock {\em IEEE Transactions on Automatic Control}, 27(4):869--879, 1982.

\bibitem{CaiLiberis2018TAC}
X. Cai and N. Bekiaris-Liberis and M. Krstic
\newblock Input-to-State Stability and Inverse Optimality of Linear Time-Varying-Delay Predictor Feedbacks.
\newblock {\em IEEE Transactions on Automatic Control}, 63(1):233--240, 2018.

\bibitem{Kharitonov2005TAC}
V. L. Kharitonov and S. -. Niculescu and J. Moreno and W. Michiels
\newblock Static output feedback stabilization: necessary conditions for multiple delay controllers.
\newblock {\em IEEE Transactions on Automatic Control}, 50(1):82--86, 2005.

\bibitem{PietriKrstic2010TAC}
D. Bresch-Pietri and M. Krstic
\newblock Delay-Adaptive Predictor Feedback for Systems With Unknown Long Actuator Delay.
\newblock {\em IEEE Transactions on Automatic Control}, 55(9):2106--2112, 2010.

\bibitem{krstic2009delay}
Krstic, Miroslav, {\em Delay compensation for nonlinear, adaptive, and PDE systems},
\newblock Springer, 2009.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\bibitem{MCRUER1980237}
D.~McRuer, ``Human dynamics in man-machine systems,'' {\em Automatica}, 16(3):237 -- 253, 1980.

\bibitem{Ross1969}
D.~Ross and I.~Fl\"{u}gge-Lotz, ``An optimal control problem for systems with
  differential-difference equation dynamics,'' {\em SIAM Journal on Control}, 7(4):609--623, 1969.

\bibitem{BASIN2007830}
M.~Basin, J.~Rodriguez-Gonzalez, and L.~Fridman, ``Optimal and robust control
  for linear state-delay systems,'' {\em Journal of the Franklin Institute}, 344(6):830 -- 845, 2007.

\bibitem{BasinTAC2006}
M.~{Basin} and J.~{Rodriguez-Gonzalez}, ``Optimal control for linear systems
  with multiple time delays in control input,'' {\em IEEE Transactions on Automatic Control}, 51(1):91--97, Jan 2006.

\bibitem{Maity2019}
D.~{Maity}, M.~H. {Mamduhi}, S.~{Hirche}, K.~H. {Johansson}, and J.~S. {Baras},
  ``Optimal {lqg} control under delay-dependent costly information,'' {\em IEEE Control Systems Letters}, 3(1):102--107, Jan 2019.

\bibitem{VRABIE2009IRL}
D.~Vrabie, O.~Pastravanu, M.~Abu-Khalaf, and F.~Lewis, ``Adaptive optimal
  control for continuous-time linear systems based on policy iteration,'' {\em Automatica}, 45(2):477 -- 484, 2009.

\bibitem{Kiumarsi2018}
B.~{Kiumarsi}, K.~G. {Vamvoudakis}, H.~{Modares}, and F.~L. {Lewis}, ``Optimal and autonomous control using reinforcement learning: A survey,''
{\em IEEE Transactions on Neural Networks and Learning Systems}, 29(6),2042--2062, June 2018.

\bibitem{Narayanan2018}
V.~{Narayanan} and S.~{Jagannathan}, ``Event-triggered distributed control of
  nonlinear interconnected systems using online reinforcement learning with
  exploration,'' {\em IEEE Transactions on Cybernetics}, 48(9):,2510--2519, Sep. 2018.

\bibitem{sutton2018reinforcement}
R.~S. Sutton and A.~G. Barto, {\em Reinforcement learning: An introduction}.
\newblock MIT press, 2018.

\bibitem{littman2015reinforcement}
M.~L. Littman, ``Reinforcement learning improves behaviour from evaluative
  feedback,'' {\em Nature}, 521(7553):445, 2015.

%%%%%%%%%%%%%%%%%%%%%%%%%%%% Event Trigger  %%%%%%%%%%%%%%%%%%%%%%%%%%%
% Event Trigger
\bibitem{tabuada2007}
P. Tabuada.
\newblock Event-triggered real-time scheduling of stabilizing control tasks.
\newblock {\em IEEE Transactions on Automatic Control}, 52(9):1680--1685, 2007.

\bibitem{vamvoudakis2017q}
K.~G. Vamvoudakis and H. Ferraz.
\newblock Model-free event-triggered control algorithm for continuous-time
  linear systems with optimal performance. \newblock {\em Automatica}, 2017.

\bibitem{dyn_borg}
D.~P. Borgers, V.~S. Dolk, and W.~P. M.~H. Heemels.
\newblock Riccati-based design of event-triggered controllers for linear systems with delays.
\newblock {\em IEEE Transactions on Automatic Control}, 63(1):174 -- 188, 2018.

\bibitem{Garcia2013TAC}
E. Garcia and P. J. Antsaklis
\newblock Model-Based Event-Triggered Control for Systems With Quantization and Time-Varying Network Delays.
\newblock {\em IEEE Transactions on Automatic Control}, 58(2):422--434, 2013.

\bibitem{Vignesh2018TNNLS}
V. Narayanan and S. Jagannathan
\newblock Event-Triggered Distributed Approximate Optimal State and Output Control of Affine Nonlinear Interconnected Systems.
\newblock {\em IEEE Transactions on Neural Network and Learning Systems}, 29(7):2846--2856, 2018.

\bibitem{Karafyllis2018TAC}
I. Karafyllis and M. Krstic
\newblock Adaptive Certainty-Equivalence Control With Regulation-Triggered Finite-Time Least-Squares Identification.
\newblock {\em IEEE Transactions on Automatic Control}, 63(10):3261--3275, 2018.

\bibitem{Vignesh2019AIAA}
V. Narayanan and S. Jagannathan and R. Moghadam.
\newblock Optimality in Event-triggered Adaptive Control of Uncertain Linear Dynamical Systems.
\newblock In {\em AIAA Scitech 2019 Forum}, 2019.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Text References %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\bibitem{strang_2016}
G. Strang, {\em Introduction to Linear Algebra}.
\newblock Cambridge Press, 2016.

%\bibitem{Bhat}
%K.~{Bhat} and H.~{Koivo}, "Modal characterizations of controllability and
%  observability in time delay systems," {\em IEEE Transactions on Automatic
%  Control}, 21):292--293, April 1976.

\bibitem{lewisoptimal}
F.~L. Lewis, D.~Vrabie, and V.~L. Syrmos, {\em Optimal control}.
\newblock John Wiley \& Sons, 2012.

\bibitem{moghadamcdc2019}
R. Moghadam and S. Jagannathan,
\newblock Approximate Optimal Adaptive Control of Partially Unknown Linear Continuous-time Systems with State Delay .
\newblock Accepted In{\em 58th IEEE Conference on Decision and Control}, 2019.

\bibitem{kreindler1972conditions}
E.~Kreindler and A.~Jameson, ``Conditions for nonnegativeness of partitioned
  matrices,'' {\em IEEE Transactions on Automatic Control}, 17(1):147--148, 1972.

\bibitem{khalil2015nonlinear}
H.~K. Khalil, {\em Nonlinear control}.
\newblock Pearson New York, 2015.

\bibitem{KUCERA1972413}
V.~Ku\v{c}era, ``On nonnegative definite solutions to matrix quadratic
  equations,'' {\em Automatica}, 8(4):413 -- 423, 1972.

\bibitem{ioannou2006adaptive}
P.~Ioannou and B.~Fidan, {\em Adaptive control tutorial}, 11.
\newblock Siam, 2006.

\bibitem{VigneshIET2016}
V. Narayanan and S. Jagannathan, ``Distributed adaptive optimal regulation of uncertain large-scale interconnected systems using hybrid Q-learning approach,'' {\em IET Control Theory Applications}, 10(12):1448 -- 1457, 2016.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Image References %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\bibitem{Zhang1999geometric}
L.~Zhang and B.~Zhang, ``A geometrical representation of McCulloch-Pitts neural model and its applications,'' {\em IEEE Transactions on Neural Networks}, 10(4):925--929, 1999.

\bibitem{Hornik1991FFNN}
K.~Hornik, ``Approximation capabilities of multilayer feedforward networks,'' {\em Neural networks }, 4(2):251--257, 1991.

\bibitem{Narendra1990TNNLS}
S. Kumpati. Narendra and K. Parthasarathy, ``Multilayer discrete-time neural-net controller with guaranteed performance,'' {\em IEEE Transactions on Neural Networks }, 7(1):107--130, 1996.

\bibitem{Jag1996TNN}
S. Jagannathan and F. L. Lewis, ``Identification and control of dynamical systems using neural networks,'' {\em IEEE Transactions on Neural Networks }, 1(1):4--27, 1990.

\bibitem{Werbos1990}
P. J. Werbos, ``Backpropagation through time: what it does and how to do it,'' {\em Proceedings of the IEEE}, 78(10):1550--1560, 1990.

\bibitem{Liu2014policy}
D. Liu and Q. Wei, ``Policy iteration adaptive dynamic programming algorithm for discrete-time nonlinear systems,'' {\em IEEE Transactions on Neural Networks and Learning Systems }, 25(3):621--634, 2014.

\bibitem{Lewis1998bookNN}
F.L. Lewis and S. Jagannathan and A. Yesildirak, {\em Neural network control of robot manipulators and non-linear systems}. \newblock CRC Press, 1998.

\bibitem{Brahma2016}
P. P. Brahma and D. Wu and Y. She, `Why deep learning works: A manifold disentanglement perspective,'' {\em IEEE transactions on neural networks and learning systems }, 27(10):1997--2008, 2016.

\bibitem{Lin2017}
H. W. Lin and M. Tegmark and D. Rolnick, `Why does deep and cheap learning work so well?,'' {\em Journal of Statistical Physics }, 168(6):1223--1247, 2017.

\bibitem{Hrushikesh2016}
H. N. Mhaskar and T. Poggio, ``Deep vs. shallow networks: An approximation theory perspective,'' {\em Analysis and Applications}, 14(6):829--848, 2016.

\bibitem{Roux2010}
L. Rux and Y. Bengio, ``Deep belief networks are compact universal approximators,'' {\em Neural computation }, 22(8):2192--2207, 2010.


\bibitem{Mnih2015nature}
V. Mnih and K. Kavukcuoglu and D. Silver and A. A. Rusu and J. Veness and M.G. Bellemare and A. Graves and M. Riedmiller and A. K. Fidjeland and G. Ostrovski and S. Petersen and C. Beattie and A. Sadik and I. Antonoglou and H. King and D. Kumaran and D. Wierstra and S. Legg and D. Hassabis, ''Human-level control through deep reinforcement learning,'' {\em Nature }, 518:529--533, 2015.

\bibitem{Silver2016nature}
D. Silver and A. Huang and C.J. Maddison and A. Guez and L. Sifre and G. van den Driessche and J. Schrittwieser and I. Antonoglou and V. Panneershelvam and M. Lanctot and S. Dieleman and D. Grewe and J. Nham and N. Kalchbrenner and I. Sutskever and T. Lillicrap and M. Leach and K. Kavukcuoglu and T. Graepel and D. Hassabis , ''Mastering the game of Go with deep neural networks and tree search,'' {\em Nature }, 529:484--489, 2016.

\bibitem{Levine2016End}
S. Levine and C. Finn and T. Darrell and P. Abbeel, ''End-to-end training of deep visuomotor policies,'' {\em The Journal of Machine Learning Research  }, 17(1):1334--1373, 2016

\bibitem{Levine2018Learning}
S. Levine and P. Pastor and A. Krizhevsky and J. Ibarz and D. Quillen, ''Learning hand-eye coordination for robotic grasping with deep learning and large-scale data collection,'' {\em The International Journal of Robotics Research }, 37(4-5):421--436, 2018.

\bibitem{Krishnan2019}
R. Krishnan and S. Jagannathan and V. A. Samaranayake `Direct error-driven learning for deep neural networks with applications to big data,'' {\em IEEE transactions on neural networks and learning systems }, 1--8, 2019.

\end{thebibliography}
